"Think Before You Speak": Improving Multi-Action Dialog Policy by Planning Single-Action Dialogs

Multi-action dialog policy (MADP), which generates multiple atomic dialog actions per turn, has been widely applied in task-oriented dialog systems to provide expressive and efficient system responses. Existing MADP models usually imitate action combinations from the labeled multi-action dialog samples. Due to data limitations, they generalize poorly toward unseen dialog flows. While interactive learning and reinforcement learning algorithms can be applied to incorporate external data sources of real users and user simulators, they take significant manual effort to build and suffer from instability. To address these issues, we propose Planning Enhanced Dialog Policy (PEDP), a novel multi-task learning framework that learns single-action dialog dynamics to enhance multi-action prediction. Our PEDP method employs model-based planning for conceiving what to express before deciding the current response through simulating single-action dialogs. Experimental results on the MultiWOZ dataset demonstrate that our fully supervised learning-based method achieves a solid task success rate of 90.6%, improving 3% compared to the state-of-the-art methods.

==> s_task.tex <==

\begin{figure*}[htp]
  \includegraphics[width=\textwidth]{framework}
  \centering
  \caption{(a) The Planning-Enhanced Dialog Policy (PEDP) framework.
    It utilizes a {\em single action dialog planning} module (b) to incorporates contextually relevant contents before multi-action prediction. 
    A total of $K$ single-action dialog procedures are planned, with the $k$-th path looking ahead $N_k$ steps
    under single-action dialog dynamics.
    At each step, the discrete policy model predicts an atomic dialog action
    $a_{n}$ given the previous hidden dialog state $\bh_{n-1}$, and
    the world model, which simulates user behavior, responds to the predicted action $a_{n}$ and update the hidden dialog state from $\bh_{n-1}$ to $\bh_{n}$.}
  \label{fig:framework}
\end{figure*}

\section{Task Formulation}
We regard MADPL as a multi-label classification task, i.e., given the current dialog
state that summarizes the dialog history, we want to predict a {\em macro-action} which is a set of
independent {\em atomic dialog actions} as the current brief response.
Following~\cite{li2020rethinking}, each atomic dialog action is a concatenation of domain name, action type, and
slot name, e.g., ``hotel-inform-area''\footnote{There are 166 atomic dialog actions in total in the action space.}.


